The TALP-UPC System for the WMT Similar Language Task: Statistical vs Neural Machine Translation

Although the problem of similar language translation has been an area of research interest for many years, yet it is still far from being solved. In this paper, we study the performance of two popular approaches: statistical and neural. We conclude that both methods yield similar results; however, the performance varies depending on the language pair. While the statistical approach outperforms the neural one by a difference of 6 BLEU points for the Spanish-Portuguese language pair, the proposed neural model surpasses the statistical one by a difference of 2 BLEU points for Czech-Polish. In the former case, the language similarity (based on perplexity) is much higher than in the latter case. Additionally, we report negative results for the system combination with back-translation. Our TALP-UPC system submission won 1st place for Czech-to-Polish and 2nd place for Spanish-to-Portuguese in the official evaluation of the 1st WMT Similar Language Translation task.

==> data.tex <==
\paragraph{Training Data}
Some training datasets were used in the previous editions of the Machine Translation of News Shared Task and were updated (Europarl v9, News Commentary v14), while some corpora were newly introduced (Wiki Titles v1, JRC Acquis).

\begin{table}[!h]
\small
\centering
\caption{Europarl v9 Parallel Corpus}
\label{europarl_v9_parallel}
\begin{tabular}{c|cl|c|l}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Czech $\leftrightarrow$ Polish}} & \multicolumn{2}{c}{\textbf{Spanish $\leftrightarrow$ Portuguese}} \\ \cline{2-5} \hline
\textbf{sentences}    & \multicolumn{2}{c|}{631372}                & \multicolumn{2}{c}{1811977}                    \\ \hline
\textbf{words}        & \multicolumn{1}{c|}{12526659}   & 12641841  & \multicolumn{1}{c|}{47832025}     & 46191472     \\ \cline{2-5} \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{Wiki Titles v1 Parallel Corpus}
\label{wiki_titles_v1_parallel}
\begin{tabular}{c|cl|c|l}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Czech $\leftrightarrow$ Polish}} & \multicolumn{2}{c}{\textbf{Spanish $\leftrightarrow$ Portuguese}} \\ \cline{2-5} \hline
\textbf{sentences}    & \multicolumn{2}{c|}{248645}                & \multicolumn{2}{c}{621296}                    \\ \hline
\textbf{words}        & \multicolumn{1}{c|}{551084}   & 554335  & \multicolumn{1}{c|}{1564668}     & 1533764     \\ \cline{2-5} \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{JRC-Acquis Parallel Corpus}
\label{jrc_acquis_parallel}
\begin{tabular}{c|cl|c|l}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Czech $\leftrightarrow$ Polish}} & \multicolumn{2}{c}{\textbf{Spanish $\leftrightarrow$ Portuguese}} \\ \cline{2-5} \hline
\textbf{sentences}    & \multicolumn{2}{c|}{1311362}                & \multicolumn{2}{c}{1650126}                    \\ \hline
\textbf{words}        & \multicolumn{1}{c|}{21409363}   & 21880482  & \multicolumn{1}{c|}{35868080}     & 33474269     \\ \cline{2-5} \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{News Commentary v14 Parallel Corpus}
\label{news_commentary_v14_parallel}
\begin{tabular}{c|c|l}
\multicolumn{1}{l|}{} & \multicolumn{2}{c}{\textbf{Spanish $\leftrightarrow$ Portuguese}} \\ \hline
\textbf{sentences}    & \multicolumn{2}{c}{48168}                    \\ \hline
\textbf{words}        & \multicolumn{1}{c|}{1271324}     & 1219031     \\ \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{Europarl v9 Monolingual Corpus}
\label{europarl_v9_monolingua}
\begin{tabular}{c|c|c|c|c|l}
\multicolumn{1}{l|}{} & \textbf{Czech} & \textbf{Polish} & \textbf{Spanish} & \multicolumn{2}{c}{\textbf{Portuguese}} \\ \hline
\textbf{sentences}    & 665433         & 382726          & 2019336          & \multicolumn{2}{c}{2015290}            \\ \hline
\textbf{words}        & 13199347       & 7087267         & 52157546         & \multicolumn{2}{c}{50462045}           \\ \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{News Crawl Monolingual Corpus}
\label{news_crawl_monolingua}
\begin{tabular}{c|c|c|c|c|l}
\multicolumn{1}{l|}{} & \textbf{Czech} & \textbf{Polish} & \textbf{Spanish} & \multicolumn{2}{c}{\textbf{Portuguese}} \\ \hline
\textbf{sentences}    & 72157988         & 814754          & 43814290          & \multicolumn{2}{c}{8301536}            \\ \hline
\textbf{words}        & 1019497060       & 12370354         & 1159300825         & \multicolumn{2}{c}{160477593}           \\ \hline
\end{tabular}
\end{table}

\begin{table}[!h]
\small
\centering
\caption{News Commentary v14 Monolingual Corpus}
\label{news_commentary_v14_monolingua}
\begin{tabular}{c|c|c|c|l}
\multicolumn{1}{l|}{} & \textbf{Czech} & \textbf{Spanish} & \multicolumn{2}{c}{\textbf{Portuguese}} \\ \hline
\textbf{sentences}    & 266705         & 424063           & \multicolumn{2}{c}{59502}              \\ \hline
\textbf{words}        & 4922572        & 10724738         & \multicolumn{2}{c}{1443204}            \\ \hline
\end{tabular}
\end{table}

\paragraph{Development and Test Data}

Development set consisted of 30 TED talks with 3050 parallel sentences (50618 Czech and 45448 Polish tokens). The test set contained 30 TED talks with 3412 parallel sentences (57587 Czech and 52658 Polish tokens).
In order to create development and test sets for the Czech-Polish language pair we performed the following steps. First, we identified 539 TED talks that occurred in both languages. Next, we randomly selected 30 TED talks for the dev and 30 TED talks for the test set, which were considered not too short and not too long, having on average 158 sentences in the dev set and 164 sentences in the test set. Overall, the number of sentences was 4744 in case of the development set and 4924 in the test set. Then unique sentences were extracted and cleaning of lines containing meta-data information was performed which resulted in 4700 sentences in the dev set and 4831 sentences in the test set. Further cleaning (using \texttt{clean-corpus-n.perl} from the \texttt{Moses}\footnote{https://github.com/moses-smt/mosesdecoder} toolkit) of the corpus to retain only sentences between 7 and 100 words limited the number of the sentences in the dev and test sets to 3050 and 3412 sentences respectively.

Development and test sets for Spanish-Portuguese were created from a corpus provided by AT Language Solutions. The initial dataset contained 12974 sentences (178920 Spanish and 175720 Portuguese tokens).   First, the extraction of unique sentences and cleaning of lines containing meta-data information was performed which narrowed the number of sentences to 11.7k sentences. Then cleaning of the corpus to retain only sentences between 7 and 100 words limited the number of the sentences to 6.8k. Finally, 3k randomly selected sentences were used for the dev set and other 3k random sentences were extracted to form the test set.

